MatSpectNet: Material Segmentation Network with Domain-Aware and Physically-Constrained Hyperspectral Reconstruction

Achieving accurate material segmentation for 3-channel RGB images is challenging due to the considerable variation in a material's appearance. Hyperspectral images, which are sets of spectral measurements sampled at multiple wavelengths, theoretically offer distinct information for material identification, as variations in intensity of electromagnetic radiation reflected by a surface depend on the material composition of a scene. However, existing hyperspectral datasets are impoverished regarding the number of images and material categories for the dense material segmentation task, and collecting and annotating hyperspectral images with a spectral camera is prohibitively expensive. To address this, we propose a new model, the MatSpectNet to segment materials with recovered hyperspectral images from RGB images. The network leverages the principles of colour perception in modern cameras to constrain the reconstructed hyperspectral images and employs the domain adaptation method to generalise the hyperspectral reconstruction capability from a spectral recovery dataset to material segmentation datasets. The reconstructed hyperspectral images are further filtered using learned response curves and enhanced with human perception. The performance of MatSpectNet is evaluated on the LMD dataset as well as the OpenSurfaces dataset. Our experiments demonstrate that MatSpectNet attains a 1.60% increase in average pixel accuracy and a 3.42% improvement in mean class accuracy compared with the most recent publication. The project code is attached to the supplementary material and will be published on GitHub.

==> tables/full_eva.tex <==
\begin{table}
  \centering
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{c|cccccc}
    \toprule
        Model & DBAT & ResNet-152 & ResNeSt-101 & EfficientNet-B5 & Swin-t & CAM-SegNet-DBA \\ 
        \midrule
        Asphalt & 88.66 $\pm$ 0.72 & 88.66 $\pm$ 0.17 & 94.35 $\pm$ 0.27 & 82.17 $\pm$ 2.80 & 91.83 $\pm$ 1.09 & 89.87 $\pm$ 1.94 \\ \hline
        Ceramic & 68.31 $\pm$ 1.31 & 65.29 $\pm$ 3.19 & 62.86 $\pm$ 0.67 & 73.34 $\pm$ 0.42 & 75.35 $\pm$ 0.42 & 75.01 $\pm$ 0.64 \\ \hline
        Concrete & 66.90 $\pm$ 1.07 & 50.89 $\pm$ 1.67 & 60.53 $\pm$ 2.00 & 59.36 $\pm$ 2.98 & 57.42 $\pm$ 4.88 & 69.20 $\pm$ 2.81 \\ \hline
        Fabric & 93.14 $\pm$ 0.16 & 85.53 $\pm$ 0.22 & 86.420 $\pm$ 0.92 & 85.33 $\pm$ 0.20 & 88.71 $\pm$ 0.50 & 90.79 $\pm$ 0.43\\ \hline
        Foliage & 95.35 $\pm 0.12$ & 93.55 $\pm$ 0.33 & 91.25 $\pm$ 1.16 & 88.21 $\pm$ 0.32 & 95.57 $\pm$ 0.45 & 94.04 $\pm$ 0.79 \\ \hline
        Food & 93.27 $\pm$ 0.22 & 90.27 $\pm$ 0.22 & 94.96 $\pm$ 0.34 & 95.84 $\pm$ 0.14 & 92.51 $\pm$ 0.83 & 95.19 $\pm$ 0.24 \\ \hline
        Glass & 73.27 $\pm$ 0.67 & 72.58 $\pm$ 2.50 & 68.33 $\pm$ 0.34 & 77.83 $\pm$ 0.94 & 77.95 $\pm$ 0.99 & 84.88 $\pm$ 1.11 \\ \hline
        Metal & 79.99 $\pm$ 0.51 & 75.35 $\pm$ 0.94 & 80.66 $\pm$ 0.34 & 76.67 $\pm$ 0.28 & 81.54 $\pm$ 1.36 & 81.83 $\pm$ 0.48 \\ \hline
        Paper & 73.83 $\pm$ 0.67 & 64.52 $\pm$ 2.87 & 71.14 $\pm$ 1.99 & 77.21 $\pm$ 0.13 & 63.05 $\pm$ 1.90 & 66.48 $\pm$ 1.43 \\ \hline
        Plaster & 71.43 $\pm$ 0.71 & 68.01 $\pm$ 0.53 & 78.76 $\pm$ 0.62 & 73.11 $\pm$ 0.64 & 78.12 $\pm$ 1.90 & 72.37 $\pm$ 1.03 \\ \hline
        Plastic & 50.62 $\pm$ 1.45 & 34.87 $\pm$ 1.21 & 36.07 $\pm$ 3.42 & 39.59 $\pm$ 0.64 & 51.64 $\pm$ 1.31 & 52.07 $\pm$ 2.28 \\ \hline
        Rubber & 82.61 $\pm$ 1.01 & 77.08 $\pm$ 3.61 & 79.57 $\pm$ 1.62 & 69.73 $\pm$ 0.29 & 83.48 $\pm$ 0.67 & 81.63 $\pm$ 1.79 \\ \hline
        Soil & 84.25 $\pm$ 0.50 & 73.27 $\pm$ 1.63 & 73.15 $\pm$ 2.67 & 79.73 $\pm$ 0.55 & 76.89 $\pm$ 1.11 & 80.39 $\pm$ 1.73 \\ \hline
        Stone & 86.94 $\pm$ 0.95 & 69.66 $\pm$ 1.42 & 52.12 $\pm$ 0.93 & 70.07 $\pm$ 0.76 & 73.05 $\pm$ 1.92 & 60.73 $\pm$ 2.76 \\ \hline
        Water & 97.12 $\pm$ 0.10 & 95.49 $\pm$ 0.33 & 97.54 $\pm$ 0.28 & 95.30 $\pm$ 0.32 & 95.78 $\pm$ 0.70 & 94.95 $\pm$ 0.69 \\ \hline
        Wood & 90.53 $\pm$ 0.37 & 76.05 $\pm$ 1.08 & 76.71 $\pm$ 1.23 & 86.69 $\pm$ 0.24 & 82.03 $\pm$ 1.11 & 87.63 $\pm$ 0.98 \\ \hline
        PixelAcc & 86.85 $\pm$ 0.08 & 80.68 $\pm$ 0.11 & 82.45 $\pm$ 0.20 & 83.17 $\pm$ 0.06 & 84.71 $\pm$ 0.26 & 86.12 $\pm$ 0.15 \\ \hline
        MeanAcc & 81.05 $\pm$ 0.28 & 73.87 $\pm$ 0.25 & 75.31 $\pm$ 0.29 & 76.91 $\pm$ 0.06 & 79.06 $\pm$ 0.46 & 79.85 $\pm$ 0.28 \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{Per-category performance analysis. The networks are trained five times to report the uncertainty.}
    \label{tab:per-cat-perform}
\end{table}

